Multi-task Bioassay Pre-training for Protein-ligand Binding Affinity Prediction

Protein-ligand binding affinity (PLBA) prediction is the fundamental task in drug discovery. Recently, various deep learning-based models predict binding affinity by incorporating the three-dimensional structure of protein-ligand complexes as input and achieving astounding progress. However, due to the scarcity of high-quality training data, the generalization ability of current models is still limited. In addition, different bioassays use varying affinity measurement labels (i.e., IC50, Ki, Kd), and different experimental conditions inevitably introduce systematic noise, which poses a significant challenge to constructing high-precision affinity prediction models. To address these issues, we (1) propose Multi-task Bioassay Pre-training (MBP), a pre-training framework for structure-based PLBA prediction; (2) construct a pre-training dataset called ChEMBL-Dock with more than 300k experimentally measured affinity labels and about 2.8M docked three-dimensional structures. By introducing multi-task pre-training to treat the prediction of different affinity labels as different tasks and classifying relative rankings between samples from the same bioassay, MBP learns robust and transferrable structural knowledge from our new ChEMBL-Dock dataset with varied and noisy labels. Experiments substantiate the capability of MBP as a general framework that can improve and be tailored to mainstream structure-based PLBA prediction tasks. To the best of our knowledge, MBP is the first affinity pre-training model and shows great potential for future development.

==> paper/4_preliminaries.tex <==
\section{PRELIMINARIES}
%In this section, we will formulate the protein-ligand binding affinity prediction problem and introduce some definitions used in this paper.
In this section, we start with a brief definition of the protein-ligand binding affinity prediction and the representation of molecular graphs, followed by a description of the assay and the data quality issue in ChEMBL.


\subsection{Assay and Data Quality Issue in ChEMBL}
% \cite{mendez2019chembl,Gaulton2011ChEMBLAL}
% We first give a definition about BioAssay



\jz{We need more references to endorse our arguments on the data quality issue in ChEMBL, e.g., \cite{papadatos2015activity}}
Let $d = (y, t, F, S)$ denote one data in ChEMBL, where $t$, $F$, and $S$  represent binding affinity type, protein FASTA sequence represents, and ligand SMILES sequence respectively. 
And $A_i = (d_{i1}, d_{i2}, ... )$ denotes assay $i$ consisting of $|A_i|$ data. In particular, data of the same assay have the same $F$.
ChEMBL can be notated as $\mathcal{D} = (A_1, A_2, ....) $, since the data in ChEMBL is sorted by "assays".
The labels in ChEMBL have different levels of accuracy and confidence because each assay may have different experimental conditions, perhaps in terms of solvent type, temperature, measurement method, etc.
We refer to this problem as \textit{assay bias}, which poses difficulties for us to utilize the data in ChEMBL.
As a subset of ChEMBL, \textit{assay bias} also exists in \datasetname, and our proposed pre-training method \modelname is designed to address this issue.



